Distributed Neural Representation for Reactive in situ Visualization

Implicit neural representations (INRs) have emerged as a powerful tool for compressing large-scale volume data. This opens up new possibilities for in situ visualization. However, the efficient application of INRs to distributed data remains an underexplored area. In this work, we develop a distributed volumetric neural representation and optimize it for in situ visualization. Our technique eliminates data exchanges between processes, achieving state-of-the-art compression speed, quality and ratios. Our technique also enables the implementation of an efficient strategy for caching large-scale simulation data in high temporal frequencies, further facilitating the use of reactive in situ visualization in a wider range of scientific problems. We integrate this system with the Ascent infrastructure and evaluate its performance and usability using real-world simulations.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = main.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = $(wildcard *.bib)

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all: msg pdf

arxiv: pdf clean
	zip -r main.zip *

msg:
	@echo "  This script defaults to 'make pdf'"

showdiff:
	perl -i -pe 's/\\def\\hidedelete/%!\\def\\hidedelete/g' main.tex
	find contents -name "*.tex" -exec perl -i -pe 's/%%\/\/%%DEL\{/\\del\{/g' {} \;

hidediff:
	perl -i -pe 's/%!\\def\\hidedelete/\\def\\hidedelete/g' main.tex
	find contents -name "*.tex" -exec perl -i -pe 's/\\del\{/%%\/\/%%DEL\{/g' {} \;

pdf: clean pdftex 

gs7: clean dvi ps pdf7

gs8: clean dvi ps pdf8

dvi: $(DVIFILES)

ps: $(PSFILES)

pdf7: $(PDFFILES7)

pdf8: $(PDFFILES8)

pdftex: $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi: %.tex
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
	$(RM) $*.toc.bak
# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex: %.tex
	echo "wir sind da"
	$(COPY);$(PDFTEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
	if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
	$(RM) $*.toc.bak
# Display relevant warnings
	egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps: %.dvi
#	dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#	dvips -Ppdf -G0 $< -o $@
	dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#	dvips $< -o $@

%.pdf7: %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< main.pdf
#	$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< main.pdf
#	$(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean:
	rm -f *.aux *.log *.blg *.brf *.cb *.ind *.idx *.ilg \
	*.inx *.toc *.out $(DVIFILES) $(PSFILES) main.pdf *~ *.zip \
	*.aux *.blg *.brf *.lbl *.log *.synctex.gz *.fls *.fdb_latexmk

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


# to remove unused references from the .bib file
# bibexport -o main.bib main.aux 

